An invitation to web geometry

This book was intended to serve as supporting material for a mini-course on web geometry delivered at the 27th Brazilian Mathematical Colloquium which took place at IMPA in the last week of July 2009.

==> biblio.tex <==
\clearpage
\addcontentsline{toc}{chapter}{Bibliography}

\begin{thebibliography}{99} %% length of the longest label {[Blaschke and Bol 1938]}
\thispagestyle{empty}

\bibitem{Abel} N.~Abel, {\it M\'ethode g\'en\'erale
pour trouver des functions d'une seule quantit\'e variable lorsqu'une
propri\'et\'e de ces fonctions est exprim\'ee par une \'equation
entre deux variables.}  {O\!e}uvres compl\`etes de N.H. Abel, tome 1, Grondhal Son (1981),
1--10.


\bibitem{Aczel}
J.
Acz\'{e}l, {\it
Quasigroups, nets, and nomograms.}
Advances in Math. {\bf 1} (1965), 383--450.


\bibitem{AGL} M. Akivis, V. Goldberg, and V.  Lychagin, {\it Linearizability of $d$-webs, $d\ge4$, on two-dimensional manifolds}.  Selecta Math. (N.S.)  {\bf 10}  (2004), 431--451.


\bibitem{Akivisbook}
M.  Akivis and A. Shelekhov, {\it Geometry and algebra of multidimensional three-webs}. Mathematics and its Applications  82. Kluwer Academic Publishers Group, 1992.



\bibitem{andreotti}
A. Andreotti,   {\it Th\'{e}or\`{e}mes de d\'{e}pendance alg\'{e}brique sur les espaces complexes pseudo-concaves.}
Bull. Soc. Math. France  \textbf{91}  (1963), 1--38.

\bibitem{ACGH}
E.~Arbarello, M.~Cornalba, P.~Griffiths and J.~Harris,
{\it Geometry of algebraic curves. Vol. I.}
Grundlehren der Mathematischen Wissenschaften \textbf{267}. Springer-Verlag  1985.




\bibitem{Arnold}
V.I.~Arnol'd,
{\it Geometrical methods in the theory of ordinary differential equations.}
 Grundlehren der Mathematischen Wissenschaften \textbf{250}. Springer-Verlag  1988.

\bibitem{ballico}
E. Ballico, {\it The bound of the genus for reducible curves.}
Rend. Mat. Appl.  \textbf{7} (1987), 177--179.

\bibitem{barlet}
D.~Barlet, {\it Le faisceau $\omega \sp{{\cdot}}\sb{X}$ sur un espace analytique $X$ de dimension pure.} Lecture Notes in Math. \textbf{670}, Springer  (1978).


\bibitem{Beltrami}
E. Beltrami,  {\it Resoluzione del problema: riportari i punti di una superficie sopra un piano in modo che le linee geodetische vengano rappresentante da linee rette.} Ann. Math {\bf 1} (1865), 185-204.


\bibitem{BPPV}
W.~Barth, C.~Hulek, C.~Peters  and A.~Van de Ven, {\it Compact complex surfaces.}  Springer  2004.


\bibitem{BeauvilleSchottky}
A.~Beauville, {\it
Le probl\`{e}me de Schottky et la conjecture de Novikov.}
S\'{e}minaire Bourbaki, Vol. 1986/87.
Ast\'{e}risque No. \textbf{152-153}  (1987),  101--112.

\bibitem{blaschke33}
W. Blaschke, {\it
Abz\"{a}hlungen f\"{u}r Kurvengewebe und Fl\"{a}chengewebe}. Abh. Math.  Hamb. Univ.  {\bf 9} (1933), 299--312.


\bibitem{blaschke332} W. Blaschke, {\it Textilegeometrie und
    Abelsche Integrale}. Jber. Deutsche Math.-Ver.     {\bf 43} (1933),
     87--97.



\bibitem{blaschke333} W. Blaschke, {\em \"{U}ber die Tangenten
    einer ebenen Kurve f\"{u}nfter Klasse}.
Abh. Math.  Hamb. Univ.
 {\bf 19} (1933), 313--317.









\bibitem{blaschke} W.~Blaschke,
 {\it \"Uber die Tangenten einer ebene Kurve f\"unfter Klasse.} Abh. Math.  Hamb. Univ. {\bf 9}  (1933), 313--317.

\bibitem{blaschkehowe32} W. Blaschke and  G. Howe, {\it   {\"U}ber
die Tangenten einer ebenen algebraischen Kurve}, Abh. Hambourg
   {\bf 9} (1932),  166--172.

\bibitem{BB} W.~Blaschke and  G.~Bol, {\it
Geometrie der Gewebe.} Die Grundlehren der Math. {\bf 49.}
Springer, Berlin,  1938.

\bibitem{bol32} G. Bol, {\em On $n$-webs of curves in a plane}.
  Bull. Amer. Math. Soc. {\bf 38} {(1932)},  855--857.

 \bibitem{bol34} G. Bol, {\em  Fl\"{a}chengewebe im dreidimensionalen Raum}. Abh. Math. Hamb. Univ. {\bf 10} (1934), 119--134.





\bibitem{bol36} G. Bol, {\em \"{U}ber ein bemerkenswertes F\"{u}nfgewebe
  in der Ebene}. Abh. Math.  Hamb. Univ. {\bf 11} (1936),  387--393.

\bibitem{bryant}
R. Bryant, G.  Manno and V. Matveev,
{\it
A solution of a problem of Sophus Lie: normal forms of two-dimensional metrics admitting two projective vector fields.}
Math. Ann. \textbf{340} (2008), 437--463.

\bibitem{Buzano} P. Buzano,{\it Tipi notevoli di 5-tessuti di curves piane.} Boll. Un. Mat. Ital. \textbf{1}
(1939), 7--11.

\bibitem{Buzano39} P.~Buzano, {\it Determinazione e studio di
superficie di $S_5$ le cui linee principali presentano una notevole
particolarit\`{a}.} Ann. Mat. Pura Appl. \textbf{18} (1939), 51--76.

\bibitem{Guy}
G. Casale, {\it Feuilletages singuliers de codimension un,
Groupo\"{i}de de Galois et int\'{e}grales premi\`{e}res.}
 Ann. Inst. Fourier   {\bf 56}  (2006),   735--779.


\bibitem{CL1}
V.~Cavalier and D.~Lehmann, {\it
Ordinary webs of codimension one.} Preprint arXiv:0703596v2 (2007).


\bibitem{CL2}
V.~Cavalier and D.~Lehmann, {\it
Global stucture of webs in codimension one.} Preprint arXiv:0803.2434v1 (2008).



\bibitem{CerveauMattei}
D.~Cerveau and J.-F.~Mattei, {\it Formes int\'{e}grables holomorphes singuli\`{e}res.} Ast\'{e}risque, \textbf{97}.
Soci\'{e}t\'{e} Math.  France  (1982).


\bibitem{chern1935}
S.-S. Chern, {\it  Abz\"{a}hlungen f\"{u}r Gewebe.}
Abh. Math.  Hamb. Univ.  {\bf 11} (1935), 163--170.



\bibitem{Jbr}
S.-S.~Chern  and P.~Griffiths, {\it Abel's theorem and webs.} Jahr.
Deutsch. Math.-Ver. {\bf 80} (1978),   13--110.



\bibitem{Jbr2}
S.-S.~Chern  and P.~Griffiths, {\it Corrections and addenda to our
paper:``Abel's theorem and webs".} Jahr. Deutsch. Math.-Ver.
{\bf 83} (1981), 78--83.



 \bibitem{CGpisa} S.-S. Chern and P. Griffiths, {\it
  An inequality for the rank of a web and webs of maximum rank}.
  {Ann. Scuola Norm. Sup. Pisa Cl. Sci. } {\bf 5} ({1978}),  {539--557}.




\bibitem{Chern} S.-S.~Chern, {\it  Web geometry.}  Bull. Amer. Math. Soc.
 {\bf 6} (1982), 1--8.

\bibitem{ChernB2} S.-S.~Chern, {\it The mathematical works of Wilhelm Blaschke--- an
update.}  In Wilhelm Blaschke Gesammelte Werke. Band {\bf 5} (1985) 21--23.

\bibitem{ChernB2b} S.-S.~Chern, {\it Wilhelm Blaschke and Web Geometry.}
In Wilhelm Blaschke Gesammelte Werke. Band {\bf 5} (1985), 25--27.





\bibitem{Chern92} S.-S. Chern,  {\it My mathematical education}.
In {Chern---a great geometer of the twentieth century},
    {Internat. Press} (1992),  {1--17}.

\bibitem{colmez}
P.~Colmez, {\it Arithm\'{e}tique de la fonction z\^{e}ta.} In  La fonction z\^{e}ta, Ed. \'{E}c. Polytech. Palaiseau (2003)  37--164.


\bibitem{Coxeter}
H. Coxeter, \emph{Introduction to geometry.} Reprint of the 1969 edition. Wiley Classics Library. John Wiley \& Sons, 1989.

\bibitem{dalbec}
J. Dalbec, {\it
Multisymmetric functions.}
Beitr\"{a}ge Algebra Geom. \textbf{40} (1999),  27--51.

\bibitem{damiano}
D. Damiano,
{\it Webs and characteristic forms of Grassmann manifolds.}
Amer. J. Math. \textbf{105} (1983),  1325--1345.


\bibitem{darboux80} G. Darboux, {\it Sur le contact des courbes
    et des surfaces}. Bulletin Soc. Math. France {\bf 4} (1880), 348--384.



\bibitem{dou1} A. Dou, {\it Plane four-webs}. Mem. Real Acad. Ci. Art. Barcelona {\bf 31} (1953), 133--218.


\bibitem{dou2} A. Dou, {\it Rang der ebenen $4$-Gewebe}.
Abh. Math. Sem. Univ. Hamburg {\bf 19} (1955), 149--157.



\bibitem{dou3} A. Dou, {\it The symmetric representation of hexagonal four-webs}.   Collect. Math.  {\bf 9}  (1957), 41--58.




\bibitem{taba}
D.~Fuchs and S.~Tabachnikov, {\it  Mathematical omnibus. Thirty lectures on classic mathematics.}
 Am. Math. Society, Providence, (2007).


\bibitem{airton}
A.~de~Medeiros,
{\it Singular foliations and differential $p$-forms.}
Ann. Fac. Sci. Toulouse Math.  \textbf{9} (2000), 451--466.

\bibitem{CayBac}
D.~Eisenbud, M.~Green and J.~Harris,
{\it Cayley-Bacharach theorems and conjectures.}
Bull. Amer. Math. Soc.  \textbf{33} (1996),  295--324.

\bibitem{EH100}
D.~Eisenbud and J.~Harris,
{\it On varieties of minimal degree (a centennial account).}
Proc. Sympos. Pure Math.  \textbf{46}, Amer. Math. Soc. (1987), 3--13.

\bibitem{fabrethesis} B.~Fabre,
{\it Nouvelles variations sur les th\'{e}or\`{e}mes d'Abel et de Lie}. Th\`{e}se de  Doctorat de L'Universit\'{e} Paris VI, 2000. Available at
\url{http://tel.archives-ouvertes.fr/}.

\bibitem{ferapontov} {E. Ferapontov},
    {\em Integrable systems in projective differential geometry}.
    {Kyushu J. Math.} {\bf 54} {(2000)}, {183--215}.



\bibitem{GKZ}
I.~Gelfand, M.~Kapranov and A.~Zelevinsky,
{\it Discriminants, resultants, and multidimensional determinants.}
Mathematics: Theory \& Applications. Birkh\"{a}user  1994.


\bibitem{gelfandmacpherson} I. Gelfand and  R. MacPherson, {\it Geometry in
    Grassmannians and a generalization of the dilogarithm}. Adv. in
  Math. {\bf 44} (1982),  279--312.


\bibitem{GhysP}
E.~Ghys, {\it Osculating curves}. Slides of a talk. Available at
\url{http://www.umpa.ens-lyon.fr/~ghys/Publis.html}, (2007).

\bibitem{Godbillon}
C.~Godbillon, {\it G\'{e}om\'{e}trie diff\'{e}rentielle et m\'{e}canique analytique.} Hermann  1969.

\bibitem{Goldbergbook}
V. Goldberg, {\it Theory of multicodimensional $(n + 1)$-webs}. Mathematics and its Applications {\bf 44}. Kluwer Acad.  Group, 1988.


\bibitem{grafsauer24} H. Graf and  R. Sauer, {\it \H{U}ber dreifach
    Geradensysteme}. Akad. Math.-naturwiss. Abt. (1924), 135--198.




\bibitem{griffiths}
P.~Griffiths, {\it Variations on a theorem of Abel.}  Invent. Math.  \textbf{35}  (1976), 321--390.

\bibitem{GH}
P.~Griffiths and J.~Harris,
{\it Principles of algebraic geometry.}
Pure and Applied Mathematics. Wiley-Interscience  1978.


\bibitem{GrAbel} P.~Griffiths, {\it The Legacy of Abel in Algebraic
Geometry.} In   The Legacy of Niels Henrik Abel, Springer-Verlag (2004),
179--205.

\bibitem{EHCAMG} J.~Harris, {\it Curves in projective space.
With the collaboration of David Eisenbud.} S\'{e}minaire de Math\'{e}matiques Sup\'{e}rieures \textbf{85},  Presses de l'Universit\'{e} de Montr\'{e}al (1982).




\bibitem{harris} {J. Harris}, {\it A bound on the geometric genus of projective varieties}.
   {Ann. Scuola Norm. Sup. Pisa} \textbf{8} ({1981}), {35--68}.


\bibitem{hartshorne}
R.~Hartshorne, Robin, {\it Algebraic geometry.}
Graduate Texts in Mathematics, No. \textbf{52} Springer-Verlag, 1977.

\bibitem{hartshorne'}
R. Hartshorne, {\it The genus of space curves.}  Ann. Univ. Ferrara Sez.  \textbf{40}  (1994), 207--223.

\bibitem{hartshorneCD}
R. Hartshorne,
 {\it Cohomological dimension of algebraic varieties.}  Ann. of Math.  \textbf{88}  (1968), 403--450.


\bibitem{Henaut1993} A.~H\'{e}naut,  {\it Sur la lin\'{e}arisation des tissus de $\mathbb C^2$}.  Topology  {\bf 32}  (1993),   531--542.


\bibitem{Henaut1994} A.~H\'{e}naut,  {\it Caract\'erisation des tissus de $\mathbb C^2$ dont le rang est maximal et qui sont lin\'earisables}.  Compositio Math. {\bf 94}  (1994),   247--268.


\bibitem{Henaut0} A.~H\'{e}naut, {\it Analytic web
geometry.} in  Web theory and related topics. World Scientific Publ. (2001),
6--47.


\bibitem{Henaut2004} A.~H\'{e}naut, {\it
On planar web geometry through abelian relations and connections}.
Ann. of Math. {\bf  159} (2004),  425--445.

\bibitem{Henaut2} A.~H\'{e}naut,
{\it Planar web geometry through abelian relations and
singularities.} In  Inspired by Chern, Nankai Tracts in Mathematics
\textbf{11} (2006), 269--295.







\bibitem{henkinpassare}
G.~Henkin and  M.~Passare, {\it Abelian differentials on singular varieties and variations on a theorem of {L}ie-{G}riffiths}. {Invent. Math.} {\bf 135} {(1999)}, {297--328}.


\bibitem{kleiman}
S.~Kleiman, {\it What is Abel's theorem anyway?} In The legacy of Niels Henrik Abel,  Springer (2004), 395--440.


\bibitem{Lane} E.~Lane, {\it A treatise on projective differential geometry}. University of Chicago Press 1942.

\bibitem{Lewin}
L.~Lewin, {\it Polylogarithms and associated functions.}
 North-Holland Publishing Co., New York-Amsterdam, 1981.

\bibitem{ABEL} O. Laudal, R. Piene (editors), {\it The Legacy of
    Niels Henrik Abel -- the Abel Bicentennial, Oslo, 2002}.
    Springer-Verlag, 2004.





\bibitem{Liouville}
R. Liouville, {\it
M\'{e}moire sur les invariants de certaines \'{e}quations diff\'{e}rentielles et sur leurs applications.}
J. de l'\'{E}c. Polyt. cah. LIX.  (1889), 7--76.


\bibitem{little}
J. Little, {\it Translation manifolds and the converse of Abel's theorem.}  Compositio Math.  \textbf{49}  (1983),   147--171.

\bibitem{MPP} D.~Mar\'{\i}n, J.~V.~Pereira and L.~Pirio,
{\it On planar webs with infinitesimal automorphisms.} In Inspired by
Chern, Nankai Tracts in Mathematics {\bf 11} (2006),  351-364.

\bibitem{Mihaileanu} N.  Mih\u{a}ileanu, {\it
Sur les tissus plans de premiere espece}.
Bull. Math. Soc. Roum. Sci. {\bf 43}  (1941), 23--26.

\bibitem{Mumford}
D.~Mumford,
{\it The red book of varieties and schemes.}
 Lecture Notes in Mathematics \textbf{1358}, Springer-Verlag  1999.


\bibitem{Nakai1}
I.~Nakai, {\it Web geometry and the equivalence problem of the first order partial differential equations.} In
 Web theory and related topics (Toulouse, 1996),  World Sci. Publ.  (2001), 150--204.


\bibitem{RWDN}
R.~Nickalls and R.~Dye, {\it The geometry of the discriminant of a polynomial.} The Mathematical Gazette \textbf{80} (1996), 279--285.


\bibitem{oesterle92}
J.~O\!esterl\'{e},
{\it Polylogarithmes.}
S\'{e}minaire Bourbaki, Exp. No. 762,
Ast\'{e}risque No. \textbf{216} (1993), 49--67.


\bibitem{ozkan} A.
\"Ozkan, {\it \"{U}ber die Sechseckbedingungen bei einer $n$-Kurvenwabe in der Ebene}. Abh. Math.  Univ. Hamburg  {\bf 21}  (1957), 95--98.






\bibitem{Pantazi}
A. Pantazi,   {\it
Sur la d\'{e}termination du rang d'un tissu plan}.
C. R. Acad. Sci. Roum. {\bf 2}  (1938), 108--111.





\bibitem{Popa}
G.~Pareschi and  M.~Popa, {\it
Castelnuovo theory and the geometric Schottky problem.}
J. Reine Angew. Math. \textbf{615} (2008), 25--44.



\bibitem{Pereira}
J.V.~Pereira, {\it Vector fields, invariant varieties and linear systems.}
Ann. Inst. Fourier \textbf{51} (2001),  1385--1405.







\bibitem{Bou} {J.V.~Pereira}, {\it Algebraization of Codimension one Webs.}
S\'{e}minaire Bourbaki. Vol. 2006/2007.
Ast\'{e}risque No. \textbf{317} (2008),  243--268.

\bibitem{CDQL} {J.V.~Pereira and L.~Pirio}, {\it Classification of exceptional CDQL webs on compact complex surfaces.}
Preprint arXiv:0806.3290 (2008).

\bibitem{Percy} J.V.~Pereira and P.F.~Sanchez, {\it
Transformation groups of holomorphic foliations.}
Comm. Anal. Geom. \textbf{10} (2002), 1115--1123.


\bibitem{PTese} L.~Pirio, {\it \'{E}quations
fonctionnelles  ab\'{e}liennes et g\'{e}om\'{e}trie des tissus.} Th\`{e}se de
Doctorat de l'Universit\'{e} Paris VI, 2004. Available eletronically at
\url{http://tel.archives-ouvertes.fr.}

\bibitem{crasluc} L.~Pirio, {\it Sur les tissus plans de rang maximal et le
probl\`eme de Chern.}  {C. R. Math. Acad. Sci.} {\bf 339}
(2004),  {131--136}.


\bibitem{Piriopoly} L.~Pirio, {\it  Abelian functional equations, planar web geometry and
polylogarithms.}  Selecta Math.  {\bf 11}   (2005),
 453--489.


\bibitem{PT} L.~Pirio and J.-M.~Tr\'{e}preau, {\it Tissus Plans
Exceptionnels et fonctions Th\^{e}ta.} Ann. Inst. Fourier \textbf{55}
(2005),  2209-2237.




\bibitem{PIRIOLIN} L.~Pirio, {\it Sur la lin\'earisation des tissus.} Preprint arXiv: 0811.1810v2. {To appear in L'Enseignement   Math\'{e}matique.}

\bibitem{piriorobert}
L.~Pirio and G.~Robert, {\it Unpublished manuscript}. (2005)

\bibitem{poincare}
H.~Poincar\'{e},
{\it Sur les surfaces de translation et les fonctions ab\'{e}liennes.}
Bull. Soc. Math. France \textbf{29} (1901), 61--86.


\bibitem{RipollT} O.~Ripoll, {\it G\'{e}om\'{e}trie des tissus
du plan et \'{e}quations diff\'{e}rentielles.} Th\`{e}se de Doctorat de
l'Universit\'{e} Bordeaux~1, 2005. Available eletronically at
\url{http://tel.archives-ouvertes.fr.} 

\bibitem{Ripoll} O.~Ripoll, {\it Properties of the connection associated with planar webs
and applications.}  Preprint arXiv:math.DG/0702321  (2007).


\bibitem{RobertBol}
G.~Robert, {\it Poincar\'{e} maps and Bol's Theorem}. Available eletronically at
\url{http://kyokan.ms.u-tokyo.ac.jp/~topology/GHC/data/Robert.pdf}
(2005).


\bibitem{Robert} G.~Robert, {\it Relations
fonctionnelles polylogarithmiques et tissus plans.} Pr\'{e}publication
{\bf 146} Universit\'{e} Bordeaux 1 (2002).


\bibitem{segal} S.
Segal, {\it Mathematicians under the Nazis}. Princeton University Press, Princeton,  2003.



\bibitem{Spencer}
D. Spencer, {\it Overdetermined systems of linear partial differential equations}.  Bull. Amer. Math. Soc.  {\bf 75}  (1969), 179--239.





\bibitem{Taba}
S.~Tabachnikov and  V.~Timorin, {\it Variations on the Tait-Kneser theorem}.
Available at \url{http://arxiv.org/abs/math/0602317} (2006).


\bibitem{tedeschi}
G. Tedeschi, {\it The genus of reduced space curves.}
Rend. Sem. Mat. Univ. Politec. Torino \textbf{56} (1998),  81--88.

\bibitem{Terracini37} A.~Terracini, {\it Su una
possibile particolarit\`{a} delle linee  principali di una superficie. I
i II.} Atti Accad. Naz. Lincei \textbf{26} (1937), 84--91 and
153--158.


\bibitem{thomsen27} G. Thomsen, {\it Un teoreme topologico sulle
    schiere di curve e una caratterizzazione geometrica sulle
    superficie isotermo-asintotiche}. Boll. Un. Mat. Ital. Bologna
    {\bf 6} (1927),  80--85.





\bibitem{Trepreau} J.-M.~Tr\'{e}preau, {\it
Alg\'{e}brisation des Tissus de Codimension $1$ -- La g\'{e}n\'{e}ralisation
d'un Th\'{e}or\`{e}me de Bol.} In Inspired by Chern, Nankai Tracts in
Mathematics {\bf 11} (2006), 399-433.


\bibitem{Tresse}
A. Tresse, {\it
D\'{e}termination des invariants ponctuels de l'\'{e}quation diff\'{e}rentielle ordinaire du second ordre $y'' = \omega (x,y,y').$} Leipzig. 87 S. gr. $8^\circ.$ (1896).



\bibitem{web} J. Grifone, E. Salem (editors), {\it Web theory
    and related topics}, World scientific, 2001.


\bibitem{Weimann}
M. Weimann, {\it
Trace et calcul r\'{e}siduel: une nouvelle version du th\'{e}or\`{e}me d'Abel inverse, formes ab\'{e}liennes.}
Ann. Fac. Sci. Toulouse Math. \textbf{16} (2007), 397--424.

\bibitem{wirtinger}
W. Wirtinger, {\it Lie's Translationmannigfaltigkeiten und das Abelsche Integrale}. Monatsch. Math. Phys. \textbf{46} (1938), 384--431.









\end{thebibliography} 
